TransEdge: Supporting Efficient Read Queries Across Untrusted Edge Nodes

We propose Transactional Edge (TransEdge), a distributed transaction processing system for untrusted environments such as edge computing systems. What distinguishes TransEdge is its focus on efficient support for read-only transactions. TransEdge allows reading from different partitions consistently using one round in most cases and no more than two rounds in the worst case. TransEdge design is centered around this dependency tracking scheme including the consensus and transaction processing protocols. Our performance evaluation shows that TransEdge's snapshot read-only transactions achieve an 9-24x speedup compared to current byzantine systems.

==> 03_gbft.tex <==
\section{GBFT Design}\label{sec:gbft}


In this section, we present WedgeDB's byzantine agreement component
that we call Global Byzantine Fault Tolerance (GBFT). We begin with
background on byzantine agreement and PBFT~\cite{castro1999correctness} that we are
building upon to design GBFT (Section~\ref{sub:byz-back}. (Readers
familiar with PBFT may want to skip the background section.)
%
Then, we present an overview of GBFT (Section~\ref{sub:byz-overview})
followed by the details of the protocol.

\subsection{Background: Byzantine Agreement and PBFT}
\label{sub:byz-back}

Byzantine agreement is the problem of getting a group of nodes to
reach consensus on a value in the presence of arbitrary byzantine
failures.  PBFT~\cite{castro1999practical} is a pioneering byzantine
agreement protocol that has influenced the development of byzantine
agreement protocols in the past two decades. More recently, it
continues to be influential in the context of permissioned blockchain
by being adopted by solutions such as IBM's
Hyperledger~\cite{androulaki2018hyperledger}. For these reasons, we
base our byzantine agreement component on PBFT.

The PBFT protocol is a leader-based byzantine agreement protocol. To
tolerate $f$ byzantine failures, $3f+1$ nodes are needed
(\emph{i.e.}, $n = 3f+1$). The protocol proceeds in \emph{views}, where each
view has a unique leader. For example, the leader of view 1 is node 1
and so on. The protocol is used to agree on the contents of a SMR
log, or log for short.  Every node has a copy of the log and a
committed request results in filling the same position (also called
\emph{sequence number}) in the log in all copies.

\cut{
In the normal-case operation, the leader of the current view drives
the commitment of new commands through three consecutive phases:
pre-prepare, prepare, and commit. The life-cycle of committing a
command begins with a user sending a request to commit a command to
the current view's leader. If the client is co-located with the
leader, then the request message's latency is negligible. The leader,
then, broadcasts a \textsf{pre-prepare} message to all other nodes.
The \textsf{pre-prepare} message is signed by the leader and contains
the view number, sequence number (the proposed position of the
command in the log), and the digest of the request's message (The
message itself is sent to the other nodes in parallel.) A node that
receives a \textsf{pre-prepare} message accepts it if it is authentic
(the signatures and digest are correct), the node is in the same view
as the leader, and the node has not accepted another requests with
the same view and sequence number.

If a node accepts a \textsf{pre-prepare} message from the leader, it
proceeds to the next phase and broadcasts a \textsf{prepare}
message to all other nodes including the leader. The
\textsf{prepare} message includes the same information as the
\textsf{pre-prepare} message. Each node waits to collect $2f$
\textsf{prepare} messages in addition to the \textsf{pre-prepare}
sent by the leader. Once these messages are received, the node
enters the \emph{prepared} phase. The significance of being prepared
is that the node now knows that all non-faulty nodes agree about the
contents of the message sent by the leader for that view and sequence
number. This is because even with $f$ faulty nodes, $f+1$ other nodes
have sent \textsf{prepare} messages with these contents---and they
intersect with every other group of $f+1$ non-faulty nodes.


Once a node enters the prepared state, it broadcasts a \textsf{commit}
message to all the other nodes. A prepared node waits for $2f+1$
\textsf{commit} messages (including its own) to enter the
\emph{commit} phase. Once in the commit phase, the node---assuming it
is non-faulty---considers the request committed and logs this
information in its local storage. Then, it responds with a
\textsf{reply} message to the client. The client waits for
identical \textsf{reply} messages from $f+1$ nodes before it
considers the command committed (because up to $f$ nodes might be
faulty.) 
}

The PBFT protocol proceeds in the following steps: (1)~a user sends a
request (\emph{e.g.}, a transaction) to the leader, (2)~the leader
broadcasts a \textsf{pre-prepare} message, (3)~a node that receives a
\textsf{pre-prepare} message broadcasts a \textsf{prepare} message,
(4)~a node that receives $2f$ \textsf{prepare} and a
\textsf{pre-prepare} messages enters the \emph{prepared} state. Any
two nodes in the prepared state agree on the contents of the request
from the leader---since the request has been relayed by $2f$ nodes.
Then, the prepared node broadcasts a \textsf{commit} message, (5)~a
node that receives $2f+1$ \textsf{commit} messages commits the
command locally and sends a \textsf{reply} message to the client, and
(6)~the client waits for $f+1$ \textsf{reply} messages before it
considers the command committed. 
%
All exchanged messages are signed to ensure their authenticity.

\cut{
\textbf{PBFT View Changes.}
A view change is a process for nodes to collectively move from one
view to another. Each view has a unique, predetermined, leader; view
changes are necessary for progress in the case the current view's
leader is faulty. The view change process is driven by timeout
actions. A node $I$ that does not hear from the current view leader
for a predetermined amount of time enters a \emph{view-change} phase.
In this case, $I$ broadcasts a \textsf{view-change} request to all
other nodes. The \textsf{view-change} request includes the new view
number in addition to information about the committed and prepared
requests known to $I$ (we will provide more details about this
later.)

The leader $I_v$ of a new view, $v$---that did not start
yet---collects all \textsf{view-change} messages with the view number
$v$. If $2f$ \textsf{view-change} messages with the view number $v$
are collected by $I_v$, then it announces that a new view is starting
by broadcasting a \textsf{new-view} message to all nodes. The
\textsf{new-view} message includes the new view number, a proof of
the received \textsf{view-change} requests and a summary of the
collected information about the committed and prepared requests at
other nodes (how this information is used will be presented later.) A
node that receives the \textsf{new-view} message enters the new view
number.  From that point, new requests are processed through the new
leader and view number.
}


A \emph{view change} is a process for nodes to collectively move from
one view to another. View changes are necessary for progress in the
case the current view's leader is faulty.  The view change proceeds
in two phases: First, nodes that do not hear from the leader
broadcast \textsf{view-change} requests.  Second, when the leader of
the new view collects $2f$ \textsf{view-change} messages, it
announces the new view with a \textsf{new-view} message. A node
receiving the \textsf{new-view} message enters the new view.
%
More details on how prepared requests transition from one view to
another in addition to various optimizations are presented in the
original paper~\cite{castro1999practical}.


\subsection{Motivation and Overview}
\label{sub:byz-overview}

The main challenge of using existing BFT protocols in WedgeDB is the
difference in system models. In existing BFT protocols, the system
model consists of $3f+1$ nodes, where $f$ is a small number. Also,
these nodes are assumed to be close to each other. In WedgeDB, the
number of nodes is much larger---proportional to the number of users.
Also, these nodes are distributed across large geographic locations.
If an existing BFT protocol is used in WedgeDB, it would be
detrimental to performance. Specifically, existing BFT protocols
require communication with more than two-thirds of all nodes. In
cases where the number of edge nodes is high, this step becomes very
expensive, especially given the wide-area links connecting edge nodes. 

Given this challenge of BFT protocols, our goal is to design a BFT
protocol that allows two features:
\begin{itemize}[leftmargin=*]
\item (1)~Small quorums to commit to the SMR log. Ideally, the quorum
sizes should be proportional to the number of tolerated failures
($f$) instead of the total number of nodes ($n$).
\item (2) Utilize the trusted cloud node when it results in a better
performance. The trusted node is farther than nearby edge nodes, but
we observe that for some maintenance tasks, the tasks complexity
might outweigh the communication latency cost to the trusted node.
\end{itemize}
In the rest of this section, we propose GBFT that
achieves these two goals.




\subsection{GBFT Normal-Case Quorums}
\label{sub:quorums}

GBFT builds upon PBFT.  We aim to propose changes to PBFT without
adding to the complexity of PBFT and its implementation in an effort
to increase the potential adoption of GBFT. We find opportunities to
enhance PBFT's performance by proposing changes in parts that are
outside of the core algorithms design and implementation.
Specifically, we target proposing changes in the deployment strategy
and quorum definitions.

In GBFT, edge nodes are grouped into
clusters of $3f+1$ nodes. This grouping is managed by the trusted
cloud node that tries to group neighboring nodes together. In
normal-case operation, GBFT enforces a local view on committing data,
where the cluster that is closest to the corresponding user is the
only one that is activated\footnote{In this section, we are
presenting the case for one instance of GBFT and thus one cluster is
active at a time. In a real deployment, multiple instances of GBFT
work concurrently where each correspond to a different partition and
thus multiple clusters are active at the same time.}. With this local
view, normal-case operation proceeds as if the nodes in the cluster
are the only nodes in the deployment. Therefore, the following
becomes the new quorum definitions in GBFT. (To retain safety, we
also redefine the view-change quorums, which we present after the
normal-case operation quorums.):
%

\begin{definition}
\label{def:redefined}
\textbf{(GBFT redefined quorums)}
\begin{itemize}
%%%
  \item \emph{Prepare quorum ($Q_p$):} The prepare quorum is the set
of nodes that needs to send \textsf{prepare} messages to a node $i$
for it (node $i$) to enter the prepared phase and send a
\textsf{commit} message. In PBFT, the prepare quorum is any set of
nodes that is greater than two thirds of all nodes (the prepare
quorum is a set of $2f+1$ nodes if $n=3f+1$; more generally it is
$\frac{2n+1}{3}$ if $n\ge3f+1$). 

In GBFT, we redefine the prepare quorum that can be used by a leader
to include any set of $2f+1$ nodes in the current active cluster,
regardless of the total number of nodes $n$.
%%%
  \item \emph{Commit quorum ($Q_c$):} The commit quorum is the set of
nodes that needs to send \textsf{commit} message to a node $i$ for it
(node $i$) to enter the commit phase and send a \textsf{reply}
message back to the client. In PBFT---like the prepare quorum---the
commit quorum is any set of nodes that is greater than two thirds of
all nodes ($\frac{2n+1}{3}$).

In GBFT, we redefine the commit quorum that can be used by a leader
to include any set of $2f+1$ nodes in the current active cluster,
regardless of the total number of nodes $n$.
%%%
  \item \emph{Reply quorum ($Q_r$):} The reply quorum is the set of
nodes that needs to send \textsf{reply} messages to the client for it
(the client) to consider the request committed. In both PBFT and
GBFT, any set of $f+1$ \textsf{reply} messages (with the same
information and outcome) suffices to commit the request.
\end{itemize} 
\end{definition}


\vspace{0.08in}
\subsection{View Change Challenges}
The clustering and small quorums we defined above for GBFT increases
the complexity of view changes (changing the leader) and increases
the overhead involved in performing them. This is due to three
challenges:
%
\begin{itemize}[leftmargin=*]
\item
(1)~Since the normal-case operation quorums are small, this means
that the view change quorums will be big. Specifically, the view
change quorums must intersect \emph{all} normal-case operation quorums
to be able to capture the most recent state. This means that the view
change quorum must intersect all clusters. This makes view
changes extremely expensive, and potentially unrealistic with
scenarios with thousands of nodes across large geographic regions.
%
\item
(2)~The leader of a view in PBFT is predetermined. This means that
the view changes follow a deterministic sequence of leaders. This is
acceptable in cases where the number of nodes is small. However, in
our system model, the number of nodes is large and this limits our
control on which node or subset of nodes we like to elect as leaders.
For example, if access to a data partition moved from California to
somewhere in Oregon, we would want to elect a leader to be an edge
node in Oregon. PBFT-style view changes might lead to high overhead
in such scenarios since a potentially large number of view changes
might be needed to move from the leader in California to the leader
in Oregon.
%
\item
(3)~The quorums of a view in PBFT are predetermined. This is related
to the previous point, but in terms of the quorums that are
associated with the view. Given the large number of nodes, we would
like to have more control on which nodes constitute the quorums for a
certain view. Additionally, clients must be able to verify that these
quorums are part of the current view---otherwise, malicious nodes
might impersonate the role of the current view quorum nodes.
\end{itemize}

\subsection{Cloud Node-Driven View Change}
To overcome the challenges of the view change process, we propose
\emph{a
view change protocol that is driven by the trusted cloud node.}  Being
driven by the cloud node enables a simpler and more efficient view
change protocol. The view change protocol is similar to PBFT's view
change, with the exception that the trusted cloud node drives it
instead of the leader of the new view. The cloud node-driven view change
can be triggered in two ways. The first is similar to PBFT, where
edge nodes in the current cluster send \textsf{view-change} requests
to the trusted cloud node. If the trusted cloud node receives $2f+1$
such messages, then is starts the view change process. The second way
the view change is triggered is a unilateral decision by the trusted
cloud node. This can be due to an administrator triggering the change
or observing that access to a partition has moved elsewhere. This
unilateral decision can only be invoked with the right access
privileges (\emph{e.g.}, a message signed by the administrator private
key.)

\textbf{Choosing the new leader and quorum.}
Once the view change is triggered, the trusted cloud node chooses
the leader and quorums for the next view. The choice depends
on the type of view change. If the view change is driven by
\textsf{view-change} messages, then it is most likely that the
current leader is malicious or non-responsive. In these cases, it
suffices to maintain the same quorums and pick another leader from
the same cluster. If the view change is due to detecting a change in
the location of the corresponding partition's users, then the new
leader and cluster will be chosen to be close to the where the
partition users have moved.

\textbf{View change algorithm.}
After the choices of the new leader and quorums are made, the process
of changing the view starts. The process has two phases: a phase to
stop the old view and a phase to start the new view.
%
In the first
phase, the trusted cloud node sends a
\textsf{stop-view} message to the nodes in the old view. When a node
receives a \textsf{stop-view} message, it refrains from participating
in any communication related to the old view and sends a
\textsf{stopped-view} message (analogous to \textsf{view-change}
messages in PBFT) back to the trusted cloud node. Along
with the \textsf{stopped-view} message, the edge node sends
information about its state, including prepared requests and other
information included in typical PBFT \textsf{view-change} messages.
%
When the trusted cloud node receives $2f+1$ \textsf{stopped-view}
messages, it considers the old view stopped and proceeds to the
second phase to create the new view. The trusted cloud node
constructs a \textsf{new-view} message, similar to the
\textsf{new-view} message in PBFT. Then, it sends it to the nodes in
the new view. When a node receives a \textsf{new-view} message, it
starts operating as part of that view.


\textbf{Correctness.} We provide a discussion of the correctness of
the redefined quorums of GBFT in section~\ref{sec:safety}.





==> 0a_proofs.tex <==
\section{Correctness}
\label{sec:correctness}

Due to the space limit, we only provide high-level proof sketches
about the correctness of GBFT and TransEdge.

\begin{theorem}
GBFT guarantees safety.
\end{theorem}
\begin{proof}
GBFT inherits its safety properties from PBFT. PBFT's correctness
rely on two factors: (1)~involving $2f+1$ nodes in the pre-prepare,
prepare, and commit phases, and (2)~ensuring a sufficient
intersection between the old view and the new view during view
changes. Factor 1 is maintained in GBFT sine any cluster contains
$3f+1$ nodes and involve $2f+1$ in commitment. Factor 2 is enforced
by the cloud node that gets the state from enough nodes in the old
view and communicate with enough nodes in the new view with the
resulting state.
\end{proof}

\begin{theorem}
TransEdge read-write transactions guarantee serializability.
\end{theorem}
\begin{proof}
TransEdge's read-write transactions are serializable due to using a 2PC
layer to commit distributed transactions. A malicious node cannot
cause an inconsistency because each step of the 2PC protocol is
validated through BFT replication.
\end{proof}

\begin{theorem}
TransEdge snapshot read-only transactions guarantee serializability.
\end{theorem}
\begin{proof}
CD vectors encode dependencies between partitions. This means that
for any conflict relation between two transactions ($t_i \rightarrow
t_j$), it is guaranteed that the CD vector for $t_j$ includes a
dependency to the batch that includes $t_i$.
%
TransEdge guarantees the absence of unsatisfied dependencies.
Now, consider a read-only transaction $t_r$ and the transactions it
reads from $t_{r0}, \ldots, t_{rn}$. There are write-read edges from
each $t_{ri}$ to $t_r$. Also, there are read-write edges from $t_r$
to another set of transactions that overwrite the values $t_{w0},
\ldots, t_{wm}$. Transaction $t_r$ would lead to an inconsistency if
a conflict from $t_{wi}$ can be established to any $t_{ri}$ (because
it will introduce a cycle.) However, this is not possible, because
such a link means that $t_{ri}$ have a dependency from $t_{wi}$, and
if such a dependency exists, then the read-only transaction would
have included the batch of $t_{wi}$ and its state in the read, which
is a contradiction.
\end{proof}

\begin{theorem}
A TransEdge snapshot read-only transaction is guaranteed to terminate
after the second round.
\end{theorem}
\begin{proof}
.
\end{proof}

\section{Safety}
\label{sec:safety}

\clearpage
The following is not going to be included in the submission.
\subsection{Serializability}

In this section, we provide a proof of the serializability of
transactions in TransEdge.
\cut{
We limit the discussion to the correctness
of distributed read-only transactions as the correctness of
read-write transactions is inherited from 2PC and the correctness of
local read-only transactions is due to reading a consistent snapshot
from a partition.
}

\subsubsection{Read-Write Transactions}

We start by proving the serializability of read-write transactions.
After we develop the correctness of read-write transactions, we show
how adding read-only transactions will maintain serializability
(Section~\ref{sub:rot-proof}). We will distinguish between the full
serializability graph ($SG$) that includes both read-write and
read-only transactions, and the \emph{update} serializability graph
($SG_u$) that will only include read-write transactions. Furthermore,
we annotate each edge in $SG$ to distinguish between edges where a
read-only transaction is either a source or a destination
($\rightarrow^{ro}$), and transactions where both the source and
destination are read-write transactions ($\rightarrow^{u}$).

\begin{lemma}
\label{lem:order}
For any edge $t_i$ to $t_j$, the corresponding partition $X$ has
the \textsf{commit} record of $t_i$ before the \textsf{prepare}
record of $t_j$.
\end{lemma}
\begin{proof}
From 2PC.
Consider an edge $t_i \rightarrow^{u} t_j$,
there are three types of edges:
\begin{itemize}
  \item (1) Write-read edges ($t_i \rightarrow^{u}_{wr} t_j$): 
Transaction $t_j$ reads from $t_i$. In TransEdge, a read operation only
reads from committed transactions, hence at the time of the read, the
\textsf{commit} record of $t_i$ is in the log. Also, the
\textsf{prepare} record of a transaction is added \emph{after} all
reads were performed, hence at the time of the read, the
\textsf{prepare} record of $t_j$ is not in the log. Therefore,
$t_i$'s \textsf{commit} record is before $t_j$'s \textsf{prepare}
record.
  \item (2) Write-write edges ($t_i \rightarrow^{u}_{ww} t_j$): 
Transaction $t_j$ overwrites the value written by $t_i$. A write is
applied at the batch with the \textsf{commit} record of the
transaction. Therefore, we know that the \textsf{commit} record of
$t_i$ is before the commit record of $t_j$. Due to this, the
\textsf{prepare} record of $t_j$ cannot be before the \textsf{commit}
record of $t_i$, because 2PC would have aborted the transaction when
detecting that there is a prepared transaction ($t_i$) that conflicts
with it and did not commit yet.
  \item (3) read-write edges ($t_i \rightarrow^{u}_{rw} t_j$):
Transaction $t_j$ overwrites the value read by $t_i$. When
transaction $t_i$ prepares, TransEdge ensures that the read value is
still the same and that there are no prepared transactions that
overwrite the value. Therefore, the \textsf{prepare} record of $t_i$
is before the \textsf{prepare} record of $t_j$. Furthermore, the
\textsf{prepare} record of $t_j$ cannot be before the \textsf{commit}
record of $t_i$ because TransEdge would have detected the read from
$t_i$'s \textsf{prepare} record and aborted $t_j$. Therefore, $t_j$'s
\textsf{prepare} record is after $t_i$'s \textsf{commit} record.
\end{itemize}
\end{proof}

\begin{lemma}
\label{lem:time}
For any edge in $SG_u$ ($t_i \rightarrow^{u} t_j$), all \textsf{commit}
records of $t_i$ commit in the log of accessed partitions before any
\textsf{commit} record of $t_j$ commits in any log. 
\end{lemma}
\begin{proof}
Since we use 2PC, a \textsf{commit} record is only committed to a log
after all \textsf{prepare} records have been committed in all
accessed partitions. From Lemma~\ref{lem:order}, we know that for
each partition, the \textsf{commit} record of $t_i$ is before the
\textsf{prepare} record of $t_j$. If the last \textsf{prepare} of
$t_j$ was committed to the log at time $ts(last prepare)$, we know
that all commit records of $t_i$ were committed to the log before
that time. We also know that---due to 2PC---the \textsf{commit}
records of $t_j$ are all committed to their logs necessarily after
time $ts(last prepare)$, hence proving the lemma.
\end{proof}

\begin{lemma}
For any sequence of edges from $t_i$ to $t_j$ in $SG_u$ (\emph{i.e.},
$t_i \rightarrow^{u} \ldots \rightarrow^{u} t_j$), the
\textsf{commit} records of $t_i$ are committed before the
\textsf{commit} records of $t_j$. The edges along the path may
correspond to different partitions.
\end{lemma}
\begin{proof}
Lemma~\ref{lem:time} applied transitively to transactions from $t_i$
to $t_j$. 
\end{proof}

\begin{lemma}
No cycles in $SG_{u}$.
\end{lemma}
\begin{proof}
By contradiction, consider a cycle $t_i \rightarrow^{u} \ldots
\rightarrow^u t_i$. With the previous lemma, the \textsf{commit}
record of $t_i$ is committed to the log before its \textsf{commit}
record, which is a contradiction.
\end{proof}

\subsubsection{Read-Only Transactions}
We now prove the correctness of the full graph ($SG$) that includes
both read-write and read-only transactions. We show that by starting
from $SG_u$ and showing that adding read-only transactions, $t_r$ to the
graph will not introduce any cycles.
%
Adding $t_r$ will lead to adding two types of edge:
%
(1) write-read
($t_i \rightarrow^{ro}_{wr} t_r$) from the transactions that wrote
the items read by $t_r$ to $t_r$, and
%
(2) read-write ($t_r
\rightarrow^{ro}_{rw} t_i$) edges from $t_r$ to the transactions that
overwrites the values read by $t_r$. (There are no new write-write
edges because $t_r$ does not write any data objects.) 


\begin{lemma}
For every edge sequence $t_i \xrightarrow{x}^{ro}_{wr} t_r
\xrightarrow{x}^{ro}_{rw} t_j$, the following is true for any
partition: $t_i$'s \textsf{commit} record is committed to the log
before $t_j$'s \textsf{prepare} record.
\end{lemma}
\begin{proof}
It is necessary that there is the following edge $t_i
\xrightarrow{x}^u_{ww} t_j$. From Lemma~\ref{lem:time}, $t_i$'s
\textsf{commit} record is committed to the log
before $t_j$'s \textsf{prepare} record in all partitions, which is
what we want to prove. 
\end{proof}


\begin{lemma}
For any edge $t_i \xrightarrow{x}^{u} t_j$, assume that $t_i$'s
commit record is in batch $b_x({t_i})$ and $t_j$'s commit record is in
batch $b_x({t_j})$. Also, assume that for any other edge between $t_i$
and $t_j$ on another partition ($t_i \xrightarrow{y}^{u} t_j$), the
commit record for $t_i$ is in $b_y(t_i)$ and the commit record for
$t_j$ is in $b_y(t_j)$.
%
The following is true: the dependency vector entry
$\mathcal{V}_{b_x(t_j)}^X[Y]$ is greater than or equal to $b_y(t_i)$.
\end{lemma}
\begin{proof}
Follows directly from the protocol.
\end{proof}

\begin{lemma}
For any edge $t_i \xrightarrow{x}^{u} t_j$, assume that $t_i$'s
commit record is in batch $b_x({t_i})$ and $t_j$'s commit record is in
batch $b_x({t_j})$. Also, assume that for any other edge between $t_i$
and $t_j$ on another partition ($t_i \xrightarrow{y}^{u} t_j$), the
commit record for $t_i$ is in $b_y(t_i)$ and the commit record for
$t_j$ is in $b_y(t_j)$.
%
The following is true for a third partition $Z$: the dependency vector entry
$\mathcal{V}_{b_x(t_j)}^X[Z]$ is greater than or equal to
$\mathcal{V}_{b_y(t_i)}^X[Z]$.
\end{lemma}
\begin{proof}
Follows directly from the protocol.
\end{proof}

\begin{lemma}
For any sequence of edges $t_i \rightarrow^u \ldots \rightarrow^u
t_j$, the following is true for every partition $X$ accessed by $t_i$
and every partition $Y$ accessed by $t_j$: the dependency vector
entry $\mathcal{V}_{b_y(t_j)}^Y[X]$ is greater than or equal to
$b_x(t_i)$.
\end{lemma}
\begin{proof}
From previous two lemmas. 
\end{proof}

\begin{theorem}
Adding a new transaction $t_r$ to an acyclic $SG_u$ for TransEdge will
not result in any new cycles.
\end{theorem}
\begin{proof}
Proving by contradiction, assume that adding $t_r$ leads to a cycle
$t_r \rightarrow^{ro}_{rw} t_i \rightarrow^{u} \ldots \rightarrow^u
t_j \rightarrow^{ro}_{wr} t_r$. (if adding $t_r$
to $SG_u$ will cause a cycle, then $t_r$ is necessarily part of that
cycle.)
From Lemma~\ref{lem:}, we know that the dependency vector in any
batch $b_j$ in $Y$ where $t_j$ is committed has the value in its dependence
vector for any partition $X$ where $t_i$ is committed,
$\mathcal{V}^{Y}_{b_j}[X]$, is greater than or equal to the batch
$b_i$ where $t_i$ is committed. This means that the read-only
transaction must have included the values of batch $b_i$ at $X$,
however, this is a contradiction since there is the edge $t_r
\rightarrow^{ro}_{rw} t_i$.
\end{proof}

\begin{theorem}
Adding a new transaction $t_r$ to an acyclic $SG$ for TransEdge will
not result in any new cycles.
\end{theorem}
\begin{proof}
.
\end{proof}

\subsection{GBFT}
In this section, we discuss the safety of GBFT. In
this discussion, we utilize and refer to PBFT's safety proofs~\cite{castro1999practical,castro1999correctness} due
to the similarity between the two protocols, and since GBFT uses the
same methods as PBFT with the exception of the allocated quorums. We
found that the correctness proofs of PBFT rely on the intersection
condition guaranteed by the large $2f+1$ quorums for both
normal-operation and view changes. In the discussions that follows, we
show that although GBFT quorums are defined differently to optimize
for the wide-area case, they still uphold the intersection conditions
needed for the safety of the protocol. 

% TODO for correctness, the commitment must be on the local
% datacenter in addition to a remote one.

%\subsection{Safety}

Safety is a guarantee that no two non-faulty replicas will disagree
on the committed message in a sequence number. Let's consider the
normal-case operation first. In the normal-case operation, the
following is true:
\begin{lemma}
In normal-case operation, all non-faulty nodes agree on the contents
of the request with the same sequence number, $i$. 
\end{lemma}
\begin{proof}
We prove this by contradiction. Assume that there are two non-faulty
nodes $A$ and $B$ that both have a prepared request for sequence
number $i$ with different values: $A$ has value $v_A$ and $B$ has
value $v_B$. This means that $A$ and $B$ have each received $2f_b+1$
\textsf{prepare} messages from nodes in the leader's datacenter.
Since there are only $3f+1$ nodes in each datacenter, this means that
the quorum of \textsf{prepare} messages for $A$ and $B$ intersects in
at least a single non-faulty node, $I$. Because $I$ is non-faulty, it
cannot lie and send both the value $v_A$ to $A$ and $v_B$ to $B$.
\end{proof}
The previous lemma shows that it is not possible for two non-faulty
nodes to disagree on the value of a request for the same sequence
number. Thus, if the request commits in the same view, it cannot be
the case that non-faulty replicas would disagree on the contents of
the request.

What is more subtle is the safety of committing requests in different
views at different nodes.  It should never be the case that two nodes
disagree on the content of a committed request in sequence number
$i$:
\begin{lemma}
If a request $r$ commits at a non-faulty node $A$ with sequence
number $i$ in view $v$, then any non-faulty node $B$ that commits a
request for sequence number $i$ in a later view (\emph{i.e.}, a view
larger than $v$) will commit the request $r$.
\end{lemma}
\begin{proof}
We prove this by contradiction. Assume that the value that $B$
commits at a later view $v'$ is $r'$, where $r \neq r'$. Because $A$
commits the value $r$ in $v$, this means that there is at least $f_b+1$
non-faulty nodes in $f_d+1$ datacenters that have the request $r$
prepared in view $v$ in sequence number $i$. A leader of a view $v'$
must collect---in the view change process---the prepared requests
from $2f_b+1$ nodes in $o-f_d$ datacenters. This means that the
leader must hear from at least one non-faulty node, $I$, that have the
request $r$ prepared in sequence number $i$ for view $v$. Therefore,
node $I$ must have sent the information about $r$ in its
\textsf{view-change} message, and consequently,
the request $r$ will be part of the \textsf{new-view} message that is
sent by the view $v'$ leader. When node $B$ receives the
\textsf{new-view} message for $v'$, it will have $r$ as the value for
sequence number $i$, which is a contradiction to our first assumption
that $B$ commits $r'$ in view $v'$ in sequence number $i$. 
\end{proof}

In the previous lemma, we considered a scenario
without checkpoints; extending this proof sketch to cases with
checkpoints can be made via the same methodology used in proofing
PBFT~\cite{castro1999practical,castro1999correctness}. At a
high-level, if a request $r$ is part of a checkpoint by view $v$,
then a node will learn about it in any future view as part of the
checkpoint and will not accept any requests for sequence numbers that
are part of a valid checkpoint.





















